Taming Android Fragmentation through Lightweight Crowdsourced Testing

Android fragmentation refers to the overwhelming diversity of Android devices and OS versions. These lead to the impossibility of testing an app on every supported device, leaving a number of compatibility bugs scattered in the community and thereby resulting in poor user experiences. To mitigate this, our fellow researchers have designed various works to automatically detect such compatibility issues. However, the current state-of-the-art tools can only be used to detect specific kinds of compatibility issues (i.e., compatibility issues caused by API signature evolution), i.e., many other essential types of compatibility issues are still unrevealed. For example, customized OS versions on real devices and semantic changes of OS could lead to serious compatibility issues, which are non-trivial to be detected statically. To this end, we propose a novel, lightweight, crowdsourced testing approach, LAZYCOW, to fill this research gap and enable the possibility of taming Android fragmentation through crowdsourced efforts. Specifically, crowdsourced testing is an emerging alternative to conventional mobile testing mechanisms that allow developers to test their products on real devices to pinpoint platform-specific issues. Experimental results on thousands of test cases on real-world Android devices show that LAZYCOW is effective in automatically identifying and verifying API-induced compatibility issues. Also, after investigating the user experience through qualitative metrics, users' satisfaction provides strong evidence that LAZYCOW is useful and welcome in practice.

==> backup.tex <==
 \mf{We should cut down this paragraph as it provides too much unnecessary information.}
 \lili{agree, we can cut the following paragraph.}
AOKP~\cite{aokpandroid}, abbreviated for Android Open Kang Project, is an open-source distribution for smart devices based on the official Android mobile operating system. It is actually started by Roman Birg as a free and open-source software, with additional original and third-party code, features, and control added. AOSPA~\cite{aospawiki} is developed by paranoid Android team for smartphones and tablet computers. It provides its proprietary color engine, substratum theme and the ability to take a screenshot via three fingers' swiping. Besides, it is one of the most famous ROM in September 2015 along with CyanogenMod. 
CyanogenMod~\cite{cyanogenmod}, short for CM, is also a free and open-source distribution, with other original and third-party code added. It is actually developed with respect to rolling release development model and offers additional features, such as native theme support, privacy guard and other interface enhancements etc. 
Lineage OS~\cite{lineageoswiki} is also a free and open-source software for smart devices. It actually is the successor to the customized CyanogenMod, from which it was forked when Cyanogen Inc. announced it would shutdown the infrastructure behind the project and end the development in December 2016. As the name of Cyanogen is till retained by the Cyanogen Inc., the project changed its name to LineageOS.
OmniROM~\cite{omnirom} was started to respond to the commercialization of ROM project CyanogenMod. It tried to support as many devices as possible and add new features as often as possible. 
ResurrectionRemix~\cite{resurrection} is also known as RR and was started in 2012. Comparing with LineageOS, it complimented the large online community, updates, and customization options. 
SlimRoms~\cite{slimroms} is another open-source customized Android operating system and was started in 2012. It provides many different setting options for user interfaces in comparison with other open-source Android releases. 
Replicant~\cite{replicant} was started in middle 2010 with emphasis on replacing all propriety Android components with free-software counterparts to provide a fully free-as-in-freedom Android derivative for smartphones and table computers. It is sponsored and supported by the Free Software Foundation and the modifications concentrate on lower-level parts of Android OS, such as the Linux kernel and drivers. crDroid~\cite{crdroid} is directly forked from LineageOS and was started in late 2012 for the Samsung Galaxy S3. It enables customers to customize their installations with more than 40 options in the settings.


\begin{minipage}{0.98\linewidth}
\tiny
\vspace{5pt}
\begin{lstlisting}[caption={Example of conflict part in conflict file. \mf{In my opinion, this examples is still too simple.}}, language=java, label={lst:merge_conf_example}]
<<<<<<< HEAD
}

public void init() {
  mLeftSide = mView.findViewById(R.id.status_bar_left_side);
  mStatusIcons = mView.findViewById(R.id.statusIcons);
  mNetworkTraffic = mView.findViewById(R.id.network_traffic);
  mBattery = mView.findViewById(R.id.battery);
=======
  mLeftSide = statusBarView.findViewById(R.id.status_bar_left_side);
  mStatusIcons = statusBarView.findViewById(R.id.statusIcons);
  mBattery = statusBarView.findViewById(R.id.battery);
>>>>>>> android/master
\end{lstlisting}
\end{minipage}

%\mf{This paragraph needs rewriting. The conflict in figure Listing~\ref{lst:merge_conf_example} is too simple. We need to use a more complex example where downstream and upstream have diverging implementations for a method.}
It is quite common that merge conflicts are encountered by developers of downstream project when they are trying to merge changes from upstream project.
In this research question, we are interested in which code entities of Java file experience the merge conflict. Specifically, the conflict part belongs to which section of the Java file. To fulfill the intention of conflict code entity detection, we merge the updates in our local environment as in previous research question. The example of conflict entity in the conflict Java file is shown in Listing~\ref{lst:merge_conf_example}. Code snippet between line ``$<<<<<<<$ HEAD'' and ``======='' resides in downstream Java file while code snippet between ``======='' and ``$>>>>>>>$ android/master'' comes from upstream codebase. To determine which entity of this conflict belongs to, we first determine every single line of the Java file before the merge happen belongs to which type entity and then extract the conflict code snippet from downstream project. At last, we check the conflict part comes from which lines of code and determine the types of entities of the conflict code snippet. For example, Listing~\ref{lst:merge_conf_example} represents that there are two different methods (the first close bracket belongs to the previous method) in downstream project while the method init does not exist and only one method exists in upstream project. Developers need to resolve this conflict to finalize the merge.

\mf{\sout{This paragraph needs rewriting. When presenting the columns do not use first, second and so on. Use the header of the column \eg Merge.} Very short discussion. We should really go much deeper in the discussion of the results for each research question.}


\pei{what is the intention of this research questions? How can we define complex changes?}
\mf{\sout{This paragraph needs rewriting. There is no discussion of the results. We need to describe the results. Project /e/ should not be in the table.} What did we learn from these numbers?}
Since conflict happens all the time when developers try to bring updates from upstream repositories, we want to know how big the conflicts are. Two different metrics are involved to measure how big the conflicts. The first one is the average lines of code of the conflict snippet. As in Listing~\ref{lst:merge_conf_example}, downstream project contains seven lines of code while upstream project includes three lines of code. Besides, we also compute how many AST nodes in the conflict part for downstream and upstream respectively. To determine how many AST nodes in the conflict part, we resort to Java parser~\cite{javaparser}, which is a tool enables developers to operate with Java source code as a Java object representation (AST) in a Java environment. Since every leaf node of the AST tree contains the line number of the AST node, we first traverse every single conflict java file before the merge operation and record the ast node as well as its line number. If the conflict happens, we will try to retrieve line numbers of the conflict code in the downstream and upstream repositories. 


%With the line numbers of the conflict code snippet and the ast nodes retrieved by utilizing Java parser, we can compute the total average lines of code and number of AST nodes in the conflict part in Table~\ref{tab:line_ast_avg}.
\begin{table}[!ht]
    \centering
    \scriptsize
    \caption{Average line and ast node of conflict part based on updated java files}
    \begin{tabular}[0.80\linewidth]{c|c|c|c|c|c|c}
    \hline
        Project             &  Java   & Method  &  D.line  &  U.line  &  D.ast & U.ast \\
    \hline
        AOKP                &    49   &   78     &   9.24   &   37.59   &  7.08     &  14.47 \\
        AOSPA               &   943   &   2,193  &   25.62  &   57.59   &  8.04     &  18.42 \\
        CyanogenMod         &   390   &   924    &   26.90  &   61.05   &  14.88    &  33.22 \\
        LineageOS           &   526   &   1,159  &   23.33  &   53.09   &  13.44    &  29.81 \\
        OmniROM             &   934   &   2,288  &   26.13  &   57.66   &  8.07     &  18.91 \\
        ResurrectionRemix   &   204   &   364    &   20.78  &   45.69   &  7.84     &  19.73 \\
        SlimRoms            &   179   &   454    &   34.64  &   80.78   &  18.98    &  41.34 \\
        replicant           &   119   &   283    &   26.35  &   54.64   &  8.90     &  19.45 \\
        crdroidandroid      &   116   &   182    &   10.34  &   26.13   &  4.23     &  12.34 \\
        % /e/               &   0     &     0    &     0     &    0      &    0   \\
    \hline
    \end{tabular}
    \label{tab:line_ast_avg}
\end{table}


\subsection{\textbf{RQ6:} Do methods affected by merge conflicts lead to a higher maintenance cost?}
%Assumption: if the merge introduces a problem then the developer would need to change the merge lines again and again. Count how many times the same lines have been changed after the merge. (at the method level)
%[GOOD ONE]

%\mf{This paragraph needs rewriting.}
Since most of the merge conflicts reside in method level, in this research question, we are interested in does the conflict affected methods involve a higher maintainer cost that is developers need to spend more time to update the implementation of these conflicted methods in the following commits. To this end, we first retrieve the conflicted method in the conflicted Java files when we do merge on our local environment. Second, for every single merge operation, we retrieve the next \emph{ten} consecutive commits following the completed merge. With the help of the version control system, Git, we can reset to every commit status and check if the affected methods are changed to not. 

Fig.~\ref{fig:method_upd_ten} and Fig.~\ref{fig:method_non_upd_ten} show the overall updates of the conflict affected methods and non-affected methods in different downstream projects within ten consecutive commits. Most of the affected methods are only updated 2 to 3 times in the following ten commits, which is the same as the one does not affected by the conflict. 

\begin{figure}
    \centering
    \includegraphics[width=0.88\linewidth]{pics/method_update.pdf}
    \caption{Number of updates of the conflict affected methods.}
    \label{fig:method_upd_ten}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.88\linewidth]{pics/method_non_update.pdf}
    \caption{Number of updates of the conflict not affected methods.}
    \label{fig:method_non_upd_ten}
\end{figure}

\begin{tcolorbox}[title=\textbf{Findings (Maintenance of conflict affected methods)}, left=2pt, right=2pt,top=2pt,bottom=2pt]
Developers of downstream projects do not spend much time on maintaining the conflict affected methods in the following commits.
\end{tcolorbox}

